Evidence of extended cold molecular gas and dust halos around $\mathbf{z\sim2.3}$ Extremely Red Quasars with ALMA

Large-scale outflows are believed to be an important mechanism in the evolution of galaxies. We can determine the impact of these outflows by studying either current galaxy outflows and their effect in the galaxy or by studying the effect of past outflows on the gas surrounding the galaxy. In this work, we examine the CO(7-6), [CI]\,($^{3} \rm P_{1} \rightarrow {\rm ^3 P}_{0}$), H$_2$O 2$_{11}$--2$_{02}$ and dust continuum emission of 15 extremely red quasars (ERQs) at z$\sim$2.3 using ALMA. By investigating the radial surface brightness profiles of both the individual sources and the stacked emission, we detect extended cold gas and dust emission on scales of $\sim$14 kpc in CO(7-6), [CI](2-1), and dust continuum. This is the first time that the presence of a large amount of molecular gas was detected on large, circum-galactic medium scales around quasar host galaxies using [CI] extended emission. We estimate the dust and molecular gas mass of these halos to be 10$^{7.6}$ and 10$^{10.6}$ M$_\odot$, indicating significant dust and molecular gas reservoirs around these extreme quasars. By estimating the timescale at which this gas can reach these distances by molecular gas outflows (7-32 Myr), we conclude that these halos are a relic of past AGN or starburst activity, rather than an effect of the current episode of extreme quasar activity.

==> Tables/Extended_emission_old.tex <==
\begin{tabular}{@{}lcccccc@{}} 
\hline  
\hline  
(1) & (2) & (3) & (4) & (5) & (6) & (7)\\ 
ID &Tracer & Model & FWHM(galaxy) & FWHM(halo) & log$_{10}$($\frac{F_{\rm halo}}{F_{\rm galaxy}}$) & BIC\\ 
    &     &  & [arcsec], [kpc] & [arcsec], [kpc] & & \\
\hline  

\multirow{2}{*}{SDSS J123241}  & \multirow{2}{*}{CO(7-6)} & Single & $ 0.35 ^{+ 0.03 }_{- 0.04 }$ , $ 2.89 ^{+ 0.27 }_{- 0.31 }$ & - & - &47.8\\
                  &       & \textbf{Double} & $ 0.07 ^{+ 0.06 }_{- 0.05 }$ , $ 0.59 ^{+ 0.51 }_{- 0.4 }$ & $ 2.7 ^{+ 0.63 }_{- 0.49 }$ ,  $ 22.38 ^{+ 5.26 }_{- 4.09 }$ &  $ -3.04 ^{+ 0.22 }_{- 0.13 }$ & 24.3\\ [2pt]
\hline                          
\multirow{2}{*}{SDSS J232326} &\multirow{2}{*}{[CI]}    & Single & $ 0.56 ^{+ 0.05 }_{- 0.05 }$ , $ 4.66 ^{+ 0.4 }_{- 0.4 }$& - & - & 13.2\\
                 &        & \textbf{Double} &  $ 0.25 ^{+ 0.15 }_{- 0.17 }$ , $ 2.1 ^{+ 1.25 }_{- 1.38 }$ & $ 2.47 ^{+ 0.91 }_{- 0.64 }$ ,  $ 20.5 ^{+ 7.53 }_{- 5.32 }$ & $ -2.06 ^{+ 0.26 }_{- 0.47 }$ & 9.2\\ [2pt]
\hline
\end{tabular} 

==> Tables/Stacking_res_old.tex <==
\begin{tabular}{lc|cccc|cccc} 
    
\hline  
\hline  
     &       & \multicolumn{4}{c}{Image-based stacking} &  \multicolumn{4}{c}{uv-based stacking} \\
     (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9)\\ 
Tracer & Model & FWHM(galaxy) & FWHM(halo) & log$_{10}$($\frac{I_{\rm halo}}{I_{\rm galaxy}}$) & BIC & FWHM(galaxy) & FWHM(halo) & log$_{10}$($\frac{F_{\rm halo}}{F_{\rm galaxy}}$) & BIC\\ 
    &     &  [arcsec], [kpc] & [arcsec], [kpc] & & & [arcsec], [kpc] & [arcsec], [kpc] & \\
\hline  

\multirow{2}{*}{CO(7-6)} & Single & $ 0.4 ^{+ 0.03 }_{- 0.03 }$ , $ 3.3 ^{+ 0.24 }_{- 0.26 }$ & - & - & 29.4 & $ 0.21 ^{+ 0.01 }_{- 0.01 }$ , $ 1.76 ^{+ 0.04 }_{- 0.05 }$ & - & \\
                         & \textbf{Double} & $ 0.11 ^{+ 0.11 }_{- 0.07 }$ , $ 0.89 ^{+ 0.87 }_{- 0.61 }$ & $ 1.71 ^{+ 0.35 }_{- 0.24 }$ ,  $ 14.17 ^{+ 2.9 }_{- 2.0 }$ & $ -2.64 ^{+ 0.3 }_{- 0.21 }$ & 12.7 & $ 0.19 ^{+ 0.01 }_{- 0.01 }$ , $ 1.61 ^{+ 0.06 }_{- 0.06 }$& $ 2.3 ^{+ 0.33 }_{- 0.27 }$ , $ 19.09 ^{+ 2.77 }_{- 2.22 }$ \\ [2pt]
\hline                          
\multirow{2}{*}{[CI]}    & Single & $ 0.6 ^{+ 0.05 }_{- 0.05 }$ , $ 4.98 ^{+ 0.38 }_{- 0.41 }$ & - & - & 16.5 & $0.35 ^{+ 0.01 }_{- 0.01 }$ , $ 2.93 ^{+ 0.08 }_{- 0.1 }$ &  - & -\\
                         & \textbf{Double} &  $ 0.22 ^{+ 0.17 }_{- 0.15 }$ , $ 1.83 ^{+ 1.4 }_{- 1.28 }$ & $ 1.62 ^{+ 0.46 }_{- 0.31 }$ ,  $ 13.48 ^{+ 3.82 }_{- 2.61 }$ & $ -1.91 ^{+ 0.34 }_{- 0.42 }$ & 11.3 & $ 0.31 ^{+ 0.02 }_{- 0.02 }$ , $ 2.58 ^{+ 0.13 }_{- 0.19 }$ & $ 1.66 ^{+ 0.4 }_{- 0.34 }$ , $ 13.77 ^{+ 3.35 }_{- 2.85 }$\\ [2pt]
\hline 
\multirow{2}{*}{H$_2$O} & \textbf{Single} & $ 0.19 ^{+ 0.11 }_{- 0.12 }$ , $ 1.56 ^{+ 0.94 }_{- 1.01 }$ & - & - & 8.22\\
                        & Double &  $ 0.23 ^{+ 0.1 }_{- 0.13 }$ , $ 1.9 ^{+ 0.83 }_{- 1.05 }$& $ 1.76 ^{+ 1.12 }_{- 0.57 }$ ,  $ 14.61 ^{+ 9.27 }_{- 4.77 }$ & $ -3.15 ^{+ 0.42 }_{- 0.26 }$ & 14.7 \\ [2pt]
\hline 
\multirow{2}{*}{Dust} & Single & $ 0.41 ^{+ 0.03 }_{- 0.03 }$ , $ 3.43 ^{+ 0.26 }_{- 0.29 }$ & - & - &33.5 & $ 0.24 ^{+ 0.01 }_{- 0.01 }$ , $ 2.01 ^{+ 0.05 }_{- 0.06 }$ & - & \\
                      & \textbf{Double} & $0.15 ^{+ 0.11 }_{- 0.1 }$ , $ 1.22 ^{+ 0.91 }_{- 0.84 }$ & $ 1.99 ^{+ 0.57 }_{- 0.36 }$ ,  $ 16.5 ^{+ 4.73 }_{- 3.03 }$ & $ -2.62 ^{+ 0.29 }_{- 0.3 }$ & 19.7 & $ 0.2 ^{+ 0.01 }_{- 0.01 }$ , $ 1.63 ^{+ 0.09 }_{- 0.09 }$ & $ 1.54 ^{+ 0.21 }_{- 0.21 }$ , $ 12.79 ^{+ 1.76 }_{- 1.72 }$ &\\ [2pt]
\hline  
\end{tabular} 
